WhY shape matters: Hydrodynamics of a Y-shaped membraneless electrolyzer

A novel Y-shaped membraneless flow-through electrolyzer is introduced to achieve a homogeneous electrochemical reaction across the entire electrode in a cost-efficient cell design with effective product separation. Numerical simulations of the electrolyte flow and electrical current within the already known I- and T-shaped cells motivate the newly proposed Y-shape cell. Furthermore, a new design criterion is developed based on the balance between bubble removal and gas generation. As proof-of-concept experimental results using the Y-shaped electrolyzer are presented, showing homogeneous gas distributions across the electrode and efficient product separation by the electrolyte flow.

==> nomenclature.tex <==
%============================================================================
%%%\section*{Nomenclature}  / section heading printed by printnomenclature
%============================================================================

% Latin symbols
\nomenclature[A$s$]{\(s\)}{Distance between electrodes in \si{\metre}}
\nomenclature[A$A$]{\(A_\mathrm{e}\)}{Area of working electrode in \si{\square\metre}}
\nomenclature[A$V$]{\(\Dot{V}\)}{Volumetric flow rate of electrolyte in \si{\cubic\metre}}
\nomenclature[A$E$]{\(E_\mathrm{c}\)}{Cell voltage in \si{\volt}}
\nomenclature[A$j$]{\(j_\mathrm{a}\)}{Current density applied at electrodes in \si{\milli\ampere\per\square\centi\metre}}
\nomenclature[A$d$]{\(d\)}{Diameter in \si{\metre}}
\nomenclature[A$D$]{\(D_\mathrm{j}\)}{Depth of the junction in \si{\metre}}
\nomenclature[A$H$]{\(H_\mathrm{e}\)}{Height of the electrode in \si{\metre}}
\nomenclature[A$H$]{\(H\)}{Homogeneity index}
\nomenclature[A$C2$]{\(C_2\)}{Inertial resistance coefficient in \si{\per\metre}}
\nomenclature[A$f$]{\(f_\mathrm{l}\)}{Transverse locking factor}
\nomenclature[A$S$]{\(\boldsymbol{S}\)}{Momentum source vector in \si{\newton\per\cubic\metre}}
\nomenclature[A$Sx$]{\(S\)}{Momentum source vector component in \si{\newton\per\cubic\metre}}
%\nomenclature[A$Sx$]{\(S_x, S_y, S_z\)}{Momentum source term vector components in \si{\newton\per\cubic\metre}}
\nomenclature[A$ub$]{\(\boldsymbol{u}\)}{Velocity vector in \si{\metre\per\second}}
\nomenclature[A$u$]{\(u\)}{Velocity component in \si{\metre\per\second}}
%\nomenclature[A$ux$]{\(u_x,u_y,w_z\)}{Velocity vector components in \si{\metre\per\second}}
\nomenclature[A$x$]{\(x,y,z\)}{Spatial cell coordinates in \si{\metre}}
\nomenclature[A$D$]{\(\boldsymbol{D}\)}{Viscous loss tensor in \si{\square\metre}}
\nomenclature[A$C$]{\(\boldsymbol{C}\)}{Inertial loss tensor in \si{\square\metre}}
\nomenclature[A$pd$]{\(\Delta p\)}{Pressure drop over the electrode in \si{\pascal}}
\nomenclature[A$T$]{\(T\)}{Thickness of porous zone in \si{\metre}}
\nomenclature[A$td$]{\(\Delta t\)}{Time step in \si{\second}}
\nomenclature[A$xd$]{\(\Delta x\)}{Spatial discretization in \si{\metre}}
\nomenclature[A$Re$]{\(Re\)}{Reynolds number}

% Greek symbols
\nomenclature[Bae]{\(\alpha_\text{e}\)}{Electrode angle in \si{\degree}}
\nomenclature[Br]{\(\rho\)}{Density of electrolyte in \si{\kilo\gram\per\cubic\metre}}
\nomenclature[Bm]{\(\mu\)}{Dynamic viscosity in \si{\kilo\gram\per\metre\second}}
\nomenclature[Ba]{\(\alpha\)}{Viscous resistance coefficient in \si{\per\square\metre}}
\nomenclature[Bx]{\(\xi,\eta,\zeta\)}{Spatial electrode coordinates in \si{\metre}}

% Subscripts
\nomenclature[Cl]{l}{lower}
\nomenclature[Cu]{u}{upper}
\nomenclature[Cp]{p}{pipe}
\nomenclature[Cw]{w}{wire}
\nomenclature[Ch]{h}{hydraulically equivalent}
\nomenclature[Ci]{i}{inlet}
\nomenclature[Co]{o}{outlet}
\nomenclature[Ce]{e}{electrode}
%\nomenclature[Cx]{\(x,y,z\)}{directions in global coordinate system}
%\nomenclature[Cxi]{\(\xi,\eta,\zeta\)}{directions in electrode coordinate system}
\nomenclature[Ct]{t}{tracer particles}

\printnomenclature[2cm]
\textcolor{red}{KS: Nomenclature not updated yet.}
